DriveStats: a Mobile Platform to Frame Effective Sustainable Driving Displays

Phone applications to track vehicle information have become more common place, providing insights into fuel consumption, vehicle status, and sustainable driving behaviorsHowever, to test what resonates with drivers without deep vehicle integration requires a proper research instrument. We built DriveStats: a reusable library (and encompassing an mobile app) to monitor driving trips and display related information. By providing estimated cost/emission reductions in a goal directed framework, we demonstrate how information utility can increase over the course of a 10 day diary study with a group of North American participants. Participants were initially interested in monetary savings reported increased utility for emissions-related information with increased app usage and resulted in self-reported sustainable behavior change. The DriveStats package can be used as a research probe for a plurality of mobility studies (driving, cycling, walking, etc.) for supporting mobile transportation research.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> abstract.tex <==
% Phone applications to track vehicle information have become more common place, providing insights into fuel consumption, vehicle status, and sustainable driving behaviors.
% However, to test what resonates with drivers without deep vehicle integration requires a proper research instrument.
% We built DriveStats: a reusable library (and encompassing an mobile app) to monitor driving trips and display related information.
% By providing estimated cost/emission reductions in a goal directed framework, we demonstrate how information utility can increase over the course of a 10 day diary study with a group of North American participants.
% Participants were initially interested in monetary savings reported increased utility for emissions-related information with increased app usage and resulted in self-reported sustainable behavior change.
% The DriveStats package can be used as a research probe for a plurality of mobility studies (driving, cycling, walking, etc.) for supporting mobile transportation research.



==> sections/conclusions.tex <==
% This study finds that a utility-centered information-seeking framework~\cite{sharot2020people} can be applied to the domain of sustainable driving information and that adding goal-directed information increases the overall informational utility.
% When put into a 10-day diary study, money savings displays remain of primary interest but saw burgeoning interest in information about carbon. 
% Participants discussed the carbon displays spawning thoughts and curiosity (i.e., increasing how often they thought about carbon---an increase in cognitive utility---when applied to their daily patterns).
% Future work is needed to see if having carbon information adjacent to monetary information or collective/social goals could increase carbon literacy. 
% Further, participants of the diary study asked for enriched carbon education or applied coaching through deeper car integration; both require further investigation. 
% %Our goal is continued research in vehicular information displays and eco-friendly driving can lower carbon emissions and increase carbon literacy and monetary savings.

% % \begin{itemize}
% % \item nature framework works
% % \item people like goals
% % \item can carbon adjacent to money help
% % \item how can coaching help
% % \end{itemize}

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "../main"
% %%% End:


==> sections/discussion.tex <==
% In this study we applied a utility-centered information framework~\cite{sharot2020people} to measure peoples interest in information about sustainable driving. After measuring people's general utility for  
% We tested information displays informed by this framework in a 10-day phone app diary study to see how personal daily habits would reflect. 
% Following these studies we find considerations for framing around money, goals, and eco-friendly driving information.

% \subsection{Money as an Immediate Attractor}
% Our results clearly indicate that monetary savings are a strong driver of information utility. Results from studies 1 and 2 found that information seeking and information utility values were higher when information about costs where highlighted. Participants in Study 3 also consistently expressed their interest in fuel costs. These results are consistent with known motivators for some sustainable behaviors. Savings on fuel and reducing personal impact on climate change often top the list of motives for why Americans opt for sustainable travel options, including purchasing an electrified vehicle\footnote{\url{https://apnorc.org/wp-content/uploads/2023/04/EPIC-factsheets.pdf} Accessed September 2023.}. 
% % We build upon these motives, confirming that monetary-related information generally outshines carbon-related information in many aspects such as desirability, usefulness, pleasure, and salience in people’s minds. 
% % As we hypothesized, this preference was prevalent but especially pronounced among participants with weaker beliefs about climate change (\ref{h22}). 

% This should not be hastily interpreted to suggest that individuals are primarily driven by financial motivations or that financial incentives are the best working solution. 
% As discussed in the literature review, financial incentives can sometimes have short-lived effects and potentially dilute or undermine genuine concern for environmental issues~\cite{bergquist2023field,gneezy2011and,deci2002self, hulleman2008task}.
% However, people's preference for information about monetary rewards could be used to bootstrap interest in sustainable behavior. Previous work has shown that monetary incentives can lead to lasting sustainable behaviors if these behaviors become part of a person's personal value system~\cite{maki2016paying, li2017incentives, verplanken2022attitudes}.
% This may be particularly useful in the context of driving. Since fuel costs are proportional to tailpipe emissions, fuel savings can often be associated with lower carbon emissions. One possibility could be to leverage people's interest in cost information to highlight the environmental impact associated with cost savings. Through enough exposure, people may begin to combine the value they associate with fuel cost savings to carbon savings. 

% Cognitive research into phenomena like the mere exposure effect~\cite{bornstein2022mere} suggests that frequent exposure to objects and concepts can increase feelings of familiarity and positive affect towards those objects. A similar principle may hold for sustainable driving information. Indeed, participants in study 2 showed slightly higher desirability and importance for carbon-related goals if these were paired with fuel costs. Additionally, some participants in Study 3 reported thinking more about their carbon-related emissions, even if their primary motivation was centered around fuel costs. Together, these findings propose promising avenues for future displays to use existing biases and tendencies to shift information-seeking behavior toward sustainable topics. 

% % If people are exposed to carbon savings at the same time as fuel savings, they may learn to value information about carbon over time.

% % Study 2 and Research into effects like the mere exposure effect,  With enough exposure, 
% % Study 2 found that goal framing can enhance people's interest in learning about carbon information, suggesting that Despite being a minority, people are interested in learning more about carbon emissions and the environmental consequences of their travel choices, as evidenced in Study 3. 
% % Moreover, Study 2 illustrated that presenting goals related to reducing carbon emissions effectively enhanced people’s interest in learning. 

% \subsection{CO\textsubscript{2} Informatics}
% Recent work by Mohanty et al.~\cite{mohanty2023save} finds that CO\textsubscript{2} by weight can help push people to make more eco-friendly choices when selecting amongst a number of options (e.g., rides in a ride-sharing app or rental cars).
% However, without some kind of choice, displays that include CO\textsubscript{2} information displayed by weight leave participants asking what a kg of carbon means.  
% In addition to asking for some education, participants in our study did ask for a quasi-social comparison to others with similar cars or driving styles.  
% Social features do support the long-term use of information systems.~\cite{10.1145/1518701.1518766}  Collective action in sustainable transportation has also been shown to be an effective intervention for greener behaviors.~\cite{10.1145/3544999.3552530,mohanty2023save}  Participants in the diary study discussed the need for knowing similar collective/social numbers to compare their performance. Further, as savings add up over time, future work could ask if such collective framing could serve as an additional motivator.

% Our results also suggest that framing information in terms of goals could provide a promising way to increase people's interest or willingness to seek information about carbon. Study 2 found a strong effect of goal framing on people's interest in seeking information about carbon along with all measures of information utility (Figure~\ref{fig:fig4}). Participants in Study 3 also expressed some interest in the tallies and period-to-period comparisons of both their fuel cost and carbon emissions savings. Moreover, participant reports suggest that contextualizing carbon information around their personal data and driving habits increased the utility of carbon information's utility, specifically cognitive utility as people reported thinking more about their carbon emissions. These results suggest that providing goals around sustainable information, specifically in the context of personal data may work best to increase the utility of sustainability-related information. Future systems aiming to communicate carbon should try to find ways to engage users by providing personalized, actionable goals that could increase their interest in seeking information about sustainable behaviors. 

% % \subsection{Carbon Goals and Cost Savings}
% % More generally, framing sustainable driving information around goals Coupled with cost savings, we find evidence that carbon goals can become more desirable (\ref{h23}).
% % In study 2, participants rated carbon-related goals as being slightly more desirable and important when they were paired with information about cost savings.
% % Additionally, some participants in Study 3 reported a growing interest in carbon-related information, even if they were primarily interested in information about fuel costs.
% % These findings suggest that pairing carbon information with other information that people find more valuable may increase its utility.
% % In the diary study we also find that contextualizing carbon information around people's personal data and driving habits also seems to increase this information's utility, specifically cognitive utility as people reported thinking more about their carbon emissions.
% % %in the diary study a cognitive utility in the information's display with individual participants personal data. 
% % Diary study participants described motivations to support joining carbon and costs as unified savings. 
% % These findings suggest that there is an opportunity for future work to combine CO\textsubscript{2} goals with cost savings to increase people's interest in carbon-related information.  

% \subsection{Limitations}
% In the diary study, the app was simplified by utilizing core APIs in iOS\@. All it could provide is rough estimates from a route planner. While it was accurate enough to have some participants wonder how it worked, for others it failed to produce meaningful data (P8, P19, P22, P27, P32).
% For the population where the app was working, the estimation is not as accurate to the truth as it could have been with vehicle integration.
% A tighter integration might ensure trust which might have an important role in the joint carbon/cost goal setting if not overall.
% Nevertheless, our findings provide encouraging results that even a small amount of personalization can help increase the utility people ascribe to carbon.

% Further, the call for actionable eco-driving information suggests the need for driver coaching.  
% While general advice can be prescribed (turn on the eco mode or avoid harsh acceleration), without vehicle integration, detailed coaching is not as easily provided, especially if this coaching needs to be provided during the act of driving itself.  
% There have been attempts to proxy driving patterns from cellphone gyroscopes~\cite{7014406}; however, computing actual fuel consumption requires deeper integration.  
% P24 and P28 specifically asked for deeper integration; P28 drives for a ride-sharing service and wanted service details as well.  

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "../main"
% %%% End:


==> sections/study3.tex <==
% \subsection{Participants}
% We recruited 36 participants from the DScout usability testing platform\footnote{\url{https://www.dscout.com} Accessed April 2024.} for a 10-day diary study, offering a USD 200 incentive for completion. Participants varied across demographics, with 23 identifying as women, one as non-binary, and 12 as men, aged between 20 to 71 years. They were selected from across the U.S. to represent a balanced mix of age, gender, and driving areas. All participants were daily drivers: 69.4\% reported sometimes driving in urban areas, 72.2\% in suburban areas, and 16.7\% in rural areas. Each participant owned and regularly operated either an HEV or ICE vehicle, while drivers of PHEV and BEV were excluded from the study due to the different ways fuel costs apply to these vehicles. Educational backgrounds included 13 college graduates and 9 postgraduates, while income levels were mostly above \$50,000 annually. All participants carried iPhones with the latest iOS 16+ versions.

% \subsection{DriveStats Use and Participant Activities}
% Participants were guided through the installation of the DriveStats app, setting necessary permissions, and learning usage guidelines, including not interacting with the app while driving. They engaged with DriveStats over 10 days in the summer of 2023, completing a series of activities as part of a diary study.

% \begin{enumerate*}
%   \item\label{li:presurvey} \textbf{Pre-launch survey}: Upon recruitment,
%   participants were asked to estimate the utility they expected to get from two
%   types of information:
%   \begin{enumerate*}[label={(\alph*)}]
%   \item potential savings on fuel costs and
%   \item possible reductions in carbon emissions while driving.
%   \end{enumerate*}

%   We employed the existing survey instrument~\citep{kelly2021individual} to assess in interests in Instrumental, Hedonic, and Cognitive utilities.
% These were asked on a $-3$ to $+3$ Likert scale.
%   Participants also reported their driving styles and motivations to use self-tracking tools, which may influence their engagement with the app irrespective of information utilities. These propensities were gauged using the pre-validated Impulsive-Driving Scale~\cite{perez2015impulsive} and a set of self-tracking motivation questions~\cite{gimpel2013quantifying}. 
  
%   % We employed the existing survey instrument~\citep{kelly2021individual} to  developed to apply and validate Sharot and Sunstein's framework. The overall interest in each type of information was assessed (e.g., ``Would you want to know the carbon emissions from your driving?''; answers ranging from $-3$:``definitely don't want to know'' to $+3$: ``definitely want to know''). \textit{Instrumental Utility} was measured as the piece of information's usefulness (e.g., ``How useful would it be to know the carbon emissions from your driving?''; answers ranging from $-3$:``not useful'' to $+3$: ``very useful''). \textit{Hedonic Utility} gauged feelings anticipated from knowing, and was measured by first asking participants how they would \textit{feel} if they learned the piece of information (e.g., ``How would you feel if you got to find out the carbon emissions from your driving?''), then asking how they would \textit{feel} if they \textit{never learned} the piece of information (e.g., ``How would you feel if you never got to find out the carbon emissions from your driving?''; answers for both ranging from $-3$:``very bad'' to $+3$: ``very good''). The final score for hedonic utility was calculated by subtracting the first answer from the second, giving a final score that could range between $-6$ and $+6$. Finally, \textit{Cognitive Utility} was measured by asking how \textit{often} people thought about the different pieces of information (e.g., ``How often do you think about the carbon emissions from your driving?''; answers ranging from $-3$:``never'' to $+3$: ``very often'').
  

% \item\label{li:diary} \textbf{Diary entries}: Participants were required to submit a minimum a diary entry every two days, documenting what prompted them to check DriveStats, alongside a screenshot and a selfie-style video explaining their interest in the specific app display. Participants could submit entries as frequently as desired. 

% \item \textbf{Midpoint check-in}: A brief survey assessed the app's usefulness and any changes in driving behavior or perceptions since its use. Participants also discussed how they planned to continue using the app. 

% \item \textbf{Exit survey}: Towards the study's end, participants needed to submit at least two additional diary entries. The exit survey revisited the utility measures from the pre-launch survey, asking participants to reflect on their engagement level with DriveStats and rate their interest in receiving more detailed information on fuel costs and carbon emissions, tailored to factors like vehicle efficiency and local fuel prices. 
  
% \item \textbf{Application log}: Because the app usage data (e.g., app open events and dwell time) were stored locally on participants' phones, participants were required to copy-paste this running log into a DScout entry. Following the study, instructions were provided to delete the app. 
% \end{enumerate*}

% \subsection{App Limitations}
% The DriveStats app faced several issues during the study. Some participants could not complete the TestFlight Beta installation or accurately display location information. Those unable to install the app were disqualified, while others who encountered inaccurate location data faced trust issues with the app. Notably, one participant consistently saw incorrect locations displayed hundreds of miles away, leading to frequent checks and eventual dismissal from the study with full compensation. The app set goals based on a 3-day non-sliding window, which proved problematic as it would typically require over a month of data to establish a more stable goal. This resulted in frustration when goals would grey out due to excessive driving during the period, with the intent being not to highlight failure but to indicate an unsuccessful period. However, the messaging around this was unclear. Throughout the 10-day diary study, static information was used to coach participants on eco-driving. Several participants expressed a desire for more personalized recommendations and data visualizations to track their progress more effectively, suggesting that these features could significantly enhance the app's value.

% \section{Results}
% Out of the 36 individuals who agreed to participate in the study, three dropped out for unspecified reasons, and two were dismissed with partial compensation owing to technical issues with the app. Two other participants did not complete the final exit survey. Several others (P8, P19, P22, P27, P32) encountered glitches but were guided to complete the tasks to the best of their abilities. Ultimately, 27 participants successfully completed all required activities. 

% \subsection{Pre--Post Survey Analysis}

% % \begin{figure}
% %   \centering
% %   \begin{minipage}{0.425\textwidth}
% % \begin{table}[H]
% % \small
% % \begin{tabular}{@{}r r@{.}l r@{.}l @{[} r@{.}l@{, }r@{.}l @{]}}
% % Measure               & \multicolumn{2}{l}{$\mu$ Diff.} & \multicolumn{2}{l}{$p$-value} & \multicolumn{4}{c}{95\%CI\textsuperscript{\dag}} \\ 
% % \toprule
% % \multicolumn{9}{l}{\textbf{Fuel Cost Saving Information}}                                   \\ 
% % \midrule
% % Want to Know          & -0&29           & 0&11    & -0&65& 0&07              \\
% % Useful                & -0&35           & 0&10    & -0&78& 0&07              \\
% % Feel good to know     & -0&03           & 0&88    & -0&45& 0&39               \\
% % Feel good NOT to know & 0&35            & 0&26    & -0&28& 0&99               \\
% % Thought frequency     & 0&58            & 0&02    & \phantom{-}0&10& 1&06               \\ 
% % \midrule
% % \multicolumn{9}{l}{\textbf{Carbon Emission Reduction Information}}                                   \\ 
% % \midrule
% % Want to Know          & -0&10           & 0&75    & -0&71& 0&51               \\
% % Useful                & 0&03            & 0&93    & -0&73& 0&80               \\
% % Feel good to know     & -0&03           & 0&90    & -0&54& 0&47               \\
% % Feel good NOT to know & 0&94            & <0&001  & \phantom{-}0&34& 1&53               \\
% % Thought frequency     & 0&52            & 0&12    & -0&14& 1&17               \\ 
% % \bottomrule
% % \multicolumn{9}{r}{\textsuperscript{\dag}95\% confidence interval}
% % \end{tabular}%
% % \caption{Paired T-Test Results: Post and pre intervention measures of information utilities}\label{tab:pre-post}
% % \end{table}
% %   \end{minipage}
% %   \hfill
% %   % \begin{minipage}{0.425\textwidth}
% %   % \includegraphics[width=\columnwidth]{figures/boxes.pdf}
% %   % \caption{\label{fig:lutes} Box plots of the dwell times across all the tabs. Participants spent significantly more time on the money tab over the carbon tab ($p=0.0117$). Tabs 2 and 3 were randomized across the population to mitigate order bias.}
% %   % \Description{A box plot showing the dwell times on each tab. The IQR for money tabs exceeds the others.}
% %   % \end{minipage}
% % \end{figure}

% To quantitatively evaluate the impact of the DriveStats app on perceived information utilities, we conducted paired t-tests comparing pre-launch and exit survey responses. % (Table~\ref{tab:pre-post}).
%  The results revealed a significant increase in how often participants thought about fuel cost savings after using the app (post-pre mean = 0.58, p = 0.02, 95\% CI = [0.10, 1.06]), indicating an increased cognitive utility of this information. Other types of utilities of monetary information, such as usefulness (instrumental) or emotions (hedonic) showed no significant changes. Notably, there was a significant increase in participants' preference \textit{not} to know about potential carbon emissions reductions after the intervention (post-pre mean = 0.94, p < 0.001, 95\% CI = [0.34, 1.53]), while other utilities of \coo\ information did not change much. This may reflect growing discomfort associated with seeing carbon output data, possibly exacerbating feelings of obligation or pressure to improve, which contrasts with the anticipated desensitization through repeated exposure.

% % To understand how personal tendencies influenced post-intervention information utilities, we analyzed driving style, self-tracking motivations, cost and carbon concerns, and climate change beliefs measured in the pre-launch survey. Using regression analyses followed by stepAIC\footnote{\url{https://www.rdocumentation.org/packages/MASS/versions/7.3-60.0.1/topics/stepAIC} Accessed April 2024.} to refine our models~\cite{zhang2016variable}, we identified key factors impacting utility perceptions. 

% % Our findings show that impulsive driving style significantly decreases the perceived value of fuel cost information across instrumental ($\beta$ = -2.99, p = 0.001, 95\% CI =[-4.66, -1.33]), hedonic ($\beta$ = -3.93, p = 0.014, 95\% CI = [-6.96, -0.90]), and cognitive utilities ($\beta$ = -3.68, p < 0.001, 95\% CI = [-5.31, -2.05]). Individuals with heightened concerns about fuel costs perceive greater value in this information, as evidenced by higher instrumental ($\beta$ = 0.56, p = 0.016, 95\% CI = [0.12, 1.01]) and cognitive utility ratings ($\beta$ = 0.84, p = 0.001, 95\% CI = [0.39, 1.29]).

% % Impulsive driving style also negatively impacts the cognitive utility of carbon emissions information, reducing \coo\-related thoughts 
% % ($\beta$ = -3.53, p = 0.006, 95\% CI = [-5.94, -1.12]). Other personal propensities also influence cognitive utility ratings for carbon emissions, such as fuel cost budgeting habits ($\beta$ =
% % 0.39, p = 0.030, 95\% CI = [0.04, 0.75]), desire to save on fuel costs ($\beta$ =
% % -1.04, p = 0.003, 95\% CI = [-1.70, -0.38]), and desire to reduce personal
% % carbon outputs ($\beta$ = 1.24, p <0.001, 95\%CI =[0.70, 1.78]). The contradicting effects of fuel cost budgeting and the desire to save on fuel costs on thinking about carbon emissions underscore the complex psychological dynamics and trade-offs behind engagement with sustainability information.    

% \subsection{Dwell Time}\label{sec:dwell-time}
% In-app activity logs tracked events such as tab openings (with the \textit{Trips} tab as the default) and instances of the app moving to the background or foreground. 
% In a fully developed application, an integrated display combining all metrics would be ideal.
% For this experiment, data was separated into tabs to encourage user engagement based on perceived utility and to facilitate dwell time analysis.
% Analysis revealed that participants spent more time on the \textit{Costs} tab compared to the \textit{Carbon} tab (Median-money: 86.7s; Median-carbon: 73.4s; Wilcox $W = 121$, $p=0.0117$; Fig.~\ref{fig:lutes}). A slight display order effect was observed despite attempts to mitigate it by randomizing the order of the \textit{Costs} and \textit{Carbon} tabs. The second tab displayed during a session consistently had a longer dwell time than the third (Median-second: 80.8s; Median-third: 73.4s; Wilcox $W = 349$, $p=0.04789$), irrespective of its content.

% \subsection{Diary Entries}
% Qualitative feedback from diary entries uncovered nuances that were not highlighted as significant in the quantitative analyses.
% DriveStats tracks user trips and displays monetary and carbon data summarizing overall (from the start of the experiment), 3-day, and trip-by-trip totals.
% Beyond UI considerations, the app details costs and potential savings from eco-driving, providing tips for more the use of eco drive mode and active eco-driving practices.

% % At its core, the app calculates a user's trips and displays money and carbon information as overall sum (from the start of the study), 3-day sum, and on a trip by trip basis.
% % In a real application, an all-in-one display would be ideal.
% % For this experiment, tab separation was made to drive participants to pick a display and gauge their choice given the utility; this interface also allows for easy dwell time monitoring per tab.
% % UI aside, the app displays costs and eco-driving savings with hints on how to
% % drive in an eco-friendly way and/or encourage drivers to turn on their eco-mode
% % setting.

% \subsubsection{Eco-Driving and Eco Mode.}
% By the midpoint check-in, most participants recalled, and many reported practicing, at least one in-app eco-driving.
% However, participants noted a decline in actionable information as they continued using the app, attributing this to the static nature of the recommendations.
% They expressed a desire for more dynamic and detailed information about their driving habits.
% Enhancements such as tracking hard brakes, providing personalized driving recommendations, and offering comparisons with other drivers were suggested to increase the app's value.
% Some drivers, (P13 and P17), already considered themselves safe, conscious, and smooth drivers, before using the app.
% % Several participants discussed using their car's eco mode as a driving setting.
% Of the 14 participants discussing eco mode, 11 viewed it favorably.
% P21 discovered their car had an eco mode and started using it, while P5 and P23 reported activating eco mode became a habit midway through the study.
% % P23 noted the trade-offs between eco mode and vehicle performance when when considering the cost and carbon impact, also highlighting situational factors such as the presence of other drivers.
% % : ``[My car] isn't very good on hills. So, on routes with uphill stretches, I often turn eco mode off for better performance, especially since other drivers are close behind. I always wonder about the difference in gas costs and carbon emissions when eco-mode is off versus when it's on.''
% Conversely, P2 and P15 felt the minor savings didn't justify its use.
% P24 preferred driving in ``normal mode'' for a more enjoyable driving experience and P7 felt eco-mode would damage their vehicle.
% % ``So it kinda came out as I was talking to the dealer that eco mode messes up your engine\ldots it performs more wear and tear on the car. And since eco-mode doesn’t really save you a boatload of money, it’s not necessary.''
% These comments illustrate a range of perceptions and experiences with eco mode, from skepticism about its benefits to concerns over its impact on vehicle longevity.

% \subsubsection{Money}
% Participants showed a stronger interest in saving money over carbon. 
% At the midpoint, 18 out of 27 drivers recalled cost savings with eco mode in the greatest detail without opening the app and monetary savings were brought up by P5, P7, P9, P20, P23, P26, P29, and P31.
% The app provided various perspectives on savings, emphasizing an accumulating effect (P9, P23, P26, P29, P31).
% % P23 noted, ``A dollar fifty difference in cost\ldots over a month or six months, that could definitely add up.''
% %P31 expressed a desire to see the cumulative effect, stating, ``It's nice to quantify it over a period of time.''
% %P9 found the amounts striking saying, ``it comes to show that I'm way off\ldots That's double what my expectation was. It's become a real eye opener.''
% Similarly, P26 and P29 started to reconsider their driving habits altogether, with P26 saying, ``Understanding trip cost changes my decision, not just how I drive, but also if I would drive [at all].''
% % Further personalized information was desired: e.g, local gas prices (4 mentions) and close gas stations (3 mentions).
% % On the other hand, P7, who remained skeptical about the benefits of eco-mode due to its perceived impact on the car's engine, commented there is just not enough savings to bother changing habits.

% \subsubsection{Carbon}
% Many participants found the \coo\ tally increasingly intriguing, though some found it confusing. 
% Being curious about carbon emissions was one of the most frequently mentioned triggers for checking the app (12 mentions), along with ``after a long drive or road trip'' (15 mentions) and ``before bed'' (13 mentions). 
% Also, 13 out of 27 vividly recalled estimated carbon emissions per trip without opening the app by the study's midpoint. 
% P20 appreciated having a personal \coo\ gauge.
% %: ``It's really informative and intriguing just to have an app and a place where you can see your carbon footprint and your the difference that you're making with your own vehicle.'' 
% P14 remarked that the carbon savings were small but ``a significant amount compared to what I was expecting,'' further wondering about ``a lot of cars' incorporated savings.'' 
% P3 expressed a desire for accessible, relatable information that connects daily activities to global carbon reduction efforts.
% %: ``There's been a lot of talk about flying and everything, so I almost want to go and see, okay, how does this compare to that? Or if I walk, how much does this save? What's the impact of this much carbon? So I'm kinda interested in those numbers\ldots I hear about carbon and purchasing carbon offsets, but I never really get to see the numbers or know more about it, and this is actually really close to my daily life now''.
% % Emotional responses to learning about carbon savings were mixed among participants. P16 exemplified the positive sentiment, stating, ``As for carbon emissions, I feel better about it, but it doesn’t matter as much just because it’s hard to have a good comparison. I do like to see that I am doing my best though, so that is good.'' On the contrary, P17 highlighted the frustration that can arise from minimal savings: ``I want to know about the fuel costs and carbon emissions of my car, BUT if the information ends up consistently being negligible (no matter what I do I only end up saving a few dollars at most, my impact on the environment is inconsequential) I’ll end up feeling frustrated and ambivalent. Perhaps this information would be more useful not in the context of my current car, but during the process where I am considering purchasing or leasing my next vehicle.'' Other minor reason for feeling bad or annoyed was because ``corporations need to lower their emissions, not drivers.'' Meanwhile, P26 expressed ambivalence about the impact of their driving habits on carbon emissions, noting, ``I don't really seem to be that interested in the \coo\ output because I don't think it's that easy to control. But then when I saw the numbers, I was quite surprised at how much carbon emission a small trip even puts out, which is like, quite a lot.'' These negative sentiments align with the pre--post survey's quantitative analysis showing increased preference \textit{not} to know about potential carbon emissions reductions. % after the app use. 
% %. P12 stated, ``How much is a lot of carbon, what's not a lot of carbon? I think I have a better understanding with gas prices, like I know, oh, I saved you dollars\ldots but not so much with the carbon, so I'm just kinda monitoring and figuring it out there\ldots I think it's motivating.''
% % P33 similarly noted, ``I could have saved ten kilograms of carbon emissions in the way I drove, and I would like to learn more about that.'' 
% Not knowing what a kilogram of \coo\ is led to further inquiries
% P1 stated ``I don't know. Did I save a tree?\ldots Am I doing a good job?'' 
% Collectively, participants (like P1, P12, and P33) demonstrated a desire for more education on carbon impact~\cite{mohanty2023save}.
% Finally, on participant (P28) stated \coo\ was ``not something I'm worried about.''

% \subsubsection{Goals}
% The app set goals by displaying a running total and a summary of the past three days, alongside overall totals. If a user exceeded their previous period’s sum, a message appeared: ``You drove more than last period, try again when the current period resets.''
% The goal feature raised cognitive utility among some participants. 
% P5 expressed interest in weekly goals, noting, ``I wanted to see how much I could save in a week. It was interesting to see the potential savings over that time frame.'' P31 found the goal motivating, appreciating the breakdown of each trip’s costs and potential savings: ``reviewing the stats helped them make more sense.'' P11 pointed out that they see low instrumental utility in provided information, stating, ``for me, as a Zoomer, I don't know how much that would affect changing my driving habits'' and that statistics are ``kind of meaningless.'' However, they acknowledged finding value in the goal feature: ``one thing I actually found interesting\ldots was the last three days', like, fuel cost.'' P1 expressed dissatisfaction noting, ``I was a little disappointed that it seems, I think, the app is telling me that I drove actually too much''.

% \subsubsection{App}
% While the DriveStats app was intentionally designed with basic functionality, participant feedback provided insights that help contextualize its usage. Several participants were curious about how the app functions. P25 commented on the app's capability to track every aspect of his drives, from routes to costs and carbon emissions, expressing appreciation for the detailed information as someone who likes numbers. P29 expressed wonder and slight skepticism about the accuracy of the app's data, questioning how it could know specific details like fuel levels and vehicle maintenance, though he acknowledged the feature's potential if accurate.

% Two participants, P1 and P28, suggested improvements to the app's design. They requested that cost and carbon data be displayed on a single page for easier comparison, although this was initially separated for research purposes related to measuring user engagement (\S\ref{sec:dwell-time}). P1 hoped for future enhancements such as graphics, sounds, and animations to make the app more engaging, while P28, who drives for a rideshare app, stressed the importance of accuracy in the app's trip cost estimates, as he frequently compares these to his own calculations. Additionally, both P1 and P29 desired more interactive and coaching elements within the app. P1 sought ``actionable information'' to improve driving habits, and P29 wanted social features that would allow users to compare their performance with others driving similar vehicles over comparable distances, enhancing the community and competitive aspects of eco-driving.

% % While the app itself was designed to be basic, some feedback related to the app helps contextualize its usage.
% % Four participants wondered (P4, P16, P25, P28), how the app works.
% % P25 noted ``you know, just tracks literally, anything when I'm when I'm out driving, it gives me from where I went, how many miles you know, I drove. It gives me, you know, costs, the carbon\ldots I'm a huge, numbers guys''.
% % P29 also remarked:
% % \begin{quote}
% % ``Like, how do they know that? How do they know how much gas is in the car? How much how do they know, you know, the maintenance has been done on the car? Like, I think all those things are prevalent to being able to tell, like, what's going on with your vehicle. So I don't know. It's weird, but I think it's a pretty cool feature if it's honest''.
% % \end{quote}
% % Two participants (P1 and P28) asked if the cost and carbon could be displayed
% % on a single page. 
% % While this was a design decision for instrumentation (\S\ref{sec:dwell-time}),
% % there was a call for a smoother design from P1 who thought ``Perhaps in the future, there'll be graphics and sounds and animations to make it more exciting''.
% % P28 drives for a ride sharing app and stated ``I'm looking at the screen, I'm comparing, like, the trip amount, like, and seeing if it's accurate to my mind because, like, I know how much gas I'm spending a day''.
% % P1 and P29 asked for more coaching and ``actionable information'' (P1) to help
% % them drive better.
% % More so, P29 asked for social-like features to know ``Hey, oh, you're, like, over this much percentage compared to other people using the same car as you, driving the same distance as you''.

% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "../main"
% %%% TeX-master: "../main"
% %%% TeX-master: "../main"
% %%% TeX-master: "../main"
% %%% End:

